Image Inpainting with Learnable Feature Imputation

A regular convolution layer applying a filter in the same way over known and unknown areas causes visual artifacts in the inpainted image. Several studies address this issue with feature re-normalization on the output of the convolution. However, these models use a significant amount of learnable parameters for feature re-normalization, or assume a binary representation of the certainty of an output. We propose (layer-wise) feature imputation of the missing input values to a convolution. In contrast to learned feature re-normalization, our method is efficient and introduces a minimal number of parameters. Furthermore, we propose a revised gradient penalty for image inpainting, and a novel GAN architecture trained exclusively on adversarial loss. Our quantitative evaluation on the FDF dataset reflects that our revised gradient penalty and alternative convolution improves generated image quality significantly. We present comparisons on CelebA-HQ and Places2 to current state-of-the-art to validate our model.

==> figures/comparisons/FRRN_0.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/masked_out/1.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/masked_out/2.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/masked_out/3.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/masked_out/5.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/masked_out/6.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/masked_out/7.png}
\caption{Input}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/gated_conv/1.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/gated_conv/2.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/gated_conv/3.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/gated_conv/5.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/gated_conv/6.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/gated_conv/7.png}
\caption{GConv \cite{GatedConvolutionYu}}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/pluralistic/1.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/pluralistic/2.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/pluralistic/3.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/pluralistic/5.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/pluralistic/6.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/pluralistic/7.png}
\caption{PIC \cite{zheng2019pluralistic}}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/FRRN/1.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/FRRN/2.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/FRRN/3.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/FRRN/5.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/FRRN/6.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/FRRN/7.png}
\caption{FRRN \cite{Guo_2019}}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/result/1.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/result/2.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/result/3.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/result/5.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/result/6.png}
\includegraphics[width=\textwidth]{images/comparisons/FRRN/places2/result/7.png}
\caption{Ours}
\end{subfigure}%%
\caption{\textbf{Places2 comparison to state-of-the-art models}
Examples selected by authors of \cite{Guo_2019} (images extracted from their paper).
Results of \cite{GatedConvolutionYu,zheng2019pluralistic} generated by using their open-source code and models.
Note that the original image size is $256 \times 256$.
We recommend the reader to zoom-in on missing regions.}
\label{fig:FRRN_0}
\end{figure}

==> figures/comparisons/LBAM_0.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/1.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/2.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/3.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/4.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/5.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/6.png}
\caption{Input}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/1.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/2.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/3.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/4.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/5.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/6.png}
\caption{LBAM \cite{BidirectionalAttentionXie}}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/1.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/2.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/3.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/4.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/5.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/6.png}
\caption{GConv \cite{GatedConvolutionYu}}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/1.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/2.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/3.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/4.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/5.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/6.png}
\caption{PIC \cite{zheng2019pluralistic}}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/1.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/2.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/3.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/4.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/5.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/6.png}
\caption{Ours}
\end{subfigure}%%
\caption{\textbf{Places2 comparison to state-of-the-art models}
Examples selected by authors of \cite{BidirectionalAttentionXie} (images extracted from their supplementary material).
Results of \cite{GatedConvolutionYu,zheng2019pluralistic} generated by using their open-source code and models.
For comparisons to Patchmatch \cite{Barnes_2009}, Global \& Local Attention \cite{Iizuka_2017}, Contextual Attention \cite{ConextualAttention2018Yu}  and Partial Conv \cite{PconvLiu}, see \cite{BidirectionalAttentionXie}.
We recommend the reader to zoom-in on missing regions.
The top two rows is presented as \textbf{failure cases} by the authors of \cite{BidirectionalAttentionXie}.}
\label{fig:LBAM_0}
\end{figure}

==> figures/comparisons/LBAM_1.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/7.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/8.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/9.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/10.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/11.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/12.png}
\caption{Input}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/7.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/8.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/9.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/10.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/11.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/12.png}
\caption{LBAM \cite{BidirectionalAttentionXie}}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/7.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/8.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/9.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/10.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/11.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/12.png}
\caption{GConv \cite{GatedConvolutionYu}}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/7.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/8.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/9.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/10.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/11.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/12.png}
\caption{PIC \cite{zheng2019pluralistic}}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/7.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/8.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/9.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/10.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/11.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/12.png}
\caption{Ours}
\end{subfigure}%%
\caption{\textbf{Places2 comparison to state-of-the-art models}
Examples selected by authors of \cite{BidirectionalAttentionXie} (images extracted from their supplementary material).
Results of \cite{GatedConvolutionYu,zheng2019pluralistic} generated by using their open-source code and models.
For comparisons to Patchmatch \cite{Barnes_2009}, Global \& Local Attention \cite{Iizuka_2017}, Contextual Attention \cite{ConextualAttention2018Yu}  and Partial Conv \cite{PconvLiu}, see \cite{BidirectionalAttentionXie}.
We recommend the reader to zoom-in on missing regions.}
\label{fig:LBAM_1}
\end{figure}

==> figures/comparisons/LBAM_2.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/13.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/14.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/15.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/16.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/17.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/18.png}
\caption{Input}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/13.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/14.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/15.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/16.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/17.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/18.png}
\caption{LBAM \cite{BidirectionalAttentionXie}}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/13.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/14.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/15.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/16.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/17.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/18.png}
\caption{GConv \cite{GatedConvolutionYu}}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/13.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/14.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/15.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/16.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/17.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/18.png}
\caption{PIC \cite{zheng2019pluralistic}}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/13.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/14.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/15.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/16.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/17.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/18.png}
\caption{Ours}
\end{subfigure}%%
\caption{\textbf{Places2 comparison to state-of-the-art models}
Examples selected by authors of \cite{BidirectionalAttentionXie} (images extracted from their supplementary material).
Results of \cite{GatedConvolutionYu,zheng2019pluralistic} generated by using their open-source code and models.
For comparisons to Patchmatch \cite{Barnes_2009}, Global \& Local Attention \cite{Iizuka_2017}, Contextual Attention \cite{ConextualAttention2018Yu}  and Partial Conv \cite{PconvLiu}, see \cite{BidirectionalAttentionXie}.
We recommend the reader to zoom-in on missing regions.}
\label{fig:LBAM_2}
\end{figure}

==> figures/comparisons/LBAM_3.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/19.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/20.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/21.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/22.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/23.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/24.png}
\caption{Input}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/19.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/20.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/21.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/22.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/23.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/24.png}
\caption{LBAM \cite{BidirectionalAttentionXie}}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/19.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/20.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/21.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/22.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/23.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/24.png}
\caption{GConv \cite{GatedConvolutionYu}}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/19.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/20.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/21.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/22.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/23.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/24.png}
\caption{PIC \cite{zheng2019pluralistic}}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/19.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/20.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/21.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/22.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/23.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/24.png}
\caption{Ours}
\end{subfigure}%%
\caption{\textbf{Places2 comparison to state-of-the-art models}
Examples selected by authors of \cite{BidirectionalAttentionXie} (images extracted from their supplementary material).
Results of \cite{GatedConvolutionYu,zheng2019pluralistic} generated by using their open-source code and models.
For comparisons to Patchmatch \cite{Barnes_2009}, Global \& Local Attention \cite{Iizuka_2017}, Contextual Attention \cite{ConextualAttention2018Yu}  and Partial Conv \cite{PconvLiu}, see \cite{BidirectionalAttentionXie}.
We recommend the reader to zoom-in on missing regions.}
\label{fig:LBAM_3}
\end{figure}

==> figures/comparisons/LBAM_4.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/25.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/26.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/masked_out/27.png}
\caption{Input}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/25.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/26.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/LBAM/27.png}
\caption{LBAM \cite{BidirectionalAttentionXie}}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/25.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/26.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/gated_conv/27.png}
\caption{GConv \cite{GatedConvolutionYu}}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/25.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/26.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/pluralistic/27.png}
\caption{PIC \cite{zheng2019pluralistic}}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/25.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/26.png}
\includegraphics[width=\textwidth]{images/comparisons/LBAM/places2/result/27.png}
\caption{Ours}
\end{subfigure}%%
\caption{\textbf{Places2 comparison to state-of-the-art models}
Examples selected by authors of \cite{BidirectionalAttentionXie} (images extracted from their supplementary material).
Results of \cite{GatedConvolutionYu,zheng2019pluralistic} generated by using their open-source code and models.
For comparisons to Patchmatch \cite{Barnes_2009}, Global \& Local Attention \cite{Iizuka_2017}, Contextual Attention \cite{ConextualAttention2018Yu}  and Partial Conv \cite{PconvLiu}, see \cite{BidirectionalAttentionXie}.
We recommend the reader to zoom-in on missing regions.}
\label{fig:LBAM_4}
\end{figure}

==> figures/comparisons/celebA-HQ_0.tex <==
\begin{figure}[!ht]
\centering
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/input/1068.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/input/643.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/input/1360.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/input/1878.png}
\caption{Input}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/gated_conv/1068.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/gated_conv/643.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/gated_conv/1360.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/gated_conv/1878.png}
\caption{GatedConv \cite{GatedConvolutionYu}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/plurastic_inpainting/1068.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/plurastic_inpainting/643.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/plurastic_inpainting/1360.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/plurastic_inpainting/1878.png}
\caption{PIC \cite{zheng2019pluralistic}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/result/1068.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/result/643.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/result/1360.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/result/1878.png}
\caption{Ours}
\end{subfigure}%%
\caption{
\textbf{CelebA-HQ (Center) comparisons to state-of-the-art image inpainting.}
Results are generated using open-source code and pre-trained models from the original authors.
All examples are randomly selected.}
\label{fig:celebA-HQ_randomly_0}
\end{figure}

==> figures/comparisons/celebA-HQ_1.tex <==
\begin{figure}[!ht]
\centering
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/input/1086.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/input/1757.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/input/1289.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/input/1355.png}
\caption{Input}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/gated_conv/1086.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/gated_conv/1757.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/gated_conv/1289.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/gated_conv/1355.png}
\caption{GatedConv \cite{GatedConvolutionYu}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/plurastic_inpainting/1086.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/plurastic_inpainting/1757.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/plurastic_inpainting/1289.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/plurastic_inpainting/1355.png}
\caption{PIC \cite{zheng2019pluralistic}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/result/1086.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/result/1757.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/result/1289.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ/result/1355.png}
\caption{Ours}
\end{subfigure}%%
\caption{
\textbf{CelebA-HQ (Center) comparisons to state-of-the-art image inpainting.}
Results are generated using open-source code and pre-trained models from the original authors.
All examples are randomly selected.}
\label{fig:celebA-HQ_randomly_1}
\end{figure}

==> figures/comparisons/celebA-HQ_free_form_0.tex <==
\begin{figure}[!ht]
\centering
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/input/1397.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/input/1442.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/input/764.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/input/1674.png}
\caption{Input}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/gated_conv/1397.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/gated_conv/1442.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/gated_conv/764.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/gated_conv/1674.png}
\caption{GatedConv \cite{GatedConvolutionYu}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/plurastic_inpainting/1397.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/plurastic_inpainting/1442.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/plurastic_inpainting/764.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/plurastic_inpainting/1674.png}
\caption{PIC \cite{zheng2019pluralistic}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/result/1397.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/result/1442.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/result/764.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/result/1674.png}
\caption{Ours}
\end{subfigure}%%
\caption{
\textbf{CelebA-HQ (Free-Form) comparisons to state-of-the-art image inpainting.}
Results are generated using open-source code and pre-trained models from the original authors.
All examples are randomly selected.}
\label{fig:celebA-HQ_free_form_randomly_0}
\end{figure}

==> figures/comparisons/celebA-HQ_free_form_1.tex <==
\begin{figure}[!ht]
\centering
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/input/2023.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/input/646.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/input/558.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/input/2371.png}
\caption{Input}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/gated_conv/2023.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/gated_conv/646.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/gated_conv/558.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/gated_conv/2371.png}
\caption{GatedConv \cite{GatedConvolutionYu}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/plurastic_inpainting/2023.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/plurastic_inpainting/646.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/plurastic_inpainting/558.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/plurastic_inpainting/2371.png}
\caption{PIC \cite{zheng2019pluralistic}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/result/2023.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/result/646.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/result/558.png}
\includegraphics[width=\textwidth]{images/comparisons/celebA-HQ_free_form/result/2371.png}
\caption{Ours}
\end{subfigure}%%
\caption{
\textbf{CelebA-HQ (Free-Form) comparisons to state-of-the-art image inpainting.}
Results are generated using open-source code and pre-trained models from the original authors.
All examples are randomly selected.}
\label{fig:celebA-HQ_free_form_randomly_1}
\end{figure}

==> figures/comparisons/gated_conv_places2_0.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/masked_out/1.png}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/masked_out/2.png}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/masked_out/3.png}
\caption{Input}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/gated_conv/1.png}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/gated_conv/2.png}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/gated_conv/3.png}
\caption{GConv \cite{GatedConvolutionYu}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/pluralistic/1.png}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/pluralistic/2.png}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/pluralistic/3.png}
\caption{PIC \cite{zheng2019pluralistic}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/result/1.png}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/result/2.png}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/result/3.png}
\caption{Ours}
\end{subfigure}%%
\caption{\textbf{Places2 comparison to state-of-the-art models}
Examples selected by authors of \cite{GatedConvolutionYu} (images extracted from their official github page).
Results of \cite{zheng2019pluralistic} generated by using their open-source code and models.
Note that original image size is $512 \times 680$.
Our network and \cite{zheng2019pluralistic} expects image size of $256 \times 256$, therefore we resize the input image.
We recommend the reader to zoom-in on missing regions.}
\label{fig:gated_conv_places2_0}
\end{figure}

==> figures/comparisons/gated_conv_places2_1.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/masked_out/4.png}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/masked_out/5.png}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/masked_out/6.png}
\caption{Input}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/gated_conv/4.png}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/gated_conv/5.png}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/gated_conv/6.png}
\caption{GConv \cite{GatedConvolutionYu}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/pluralistic/4.png}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/pluralistic/5.png}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/pluralistic/6.png}
\caption{PIC \cite{zheng2019pluralistic}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/result/4.png}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/result/5.png}
\includegraphics[width=\textwidth]{images/comparisons/gated_conv/places2/result/6.png}
\caption{Ours}
\end{subfigure}%%
\caption{\textbf{Places2 comparison to state-of-the-art models}
Examples selected by authors of \cite{GatedConvolutionYu} (images extracted from their official github page).
Results of \cite{zheng2019pluralistic} generated by using their open-source code and models.
Note that original image size is $512 \times 680$.
Our network and \cite{zheng2019pluralistic} expects image size of $256 \times 256$, therefore we resize the input image.
We recommend the reader to zoom-in on missing regions.}
\label{fig:gated_conv_places2_1}
\end{figure}

==> figures/comparisons/places2_0.tex <==
\begin{figure}[!ht]
\centering
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/places2/input/642.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/input/12279.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/input/7494.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/input/28251.png}
\caption{Input}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/places2/gated_conv/642.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/gated_conv/12279.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/gated_conv/7494.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/gated_conv/28251.png}
\caption{GatedConv \cite{GatedConvolutionYu}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/places2/plurastic_inpainting/642.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/plurastic_inpainting/12279.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/plurastic_inpainting/7494.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/plurastic_inpainting/28251.png}
\caption{PIC \cite{zheng2019pluralistic}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/places2/result/642.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/result/12279.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/result/7494.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/result/28251.png}
\caption{Ours}
\end{subfigure}%%
\caption{
\textbf{Places2 (Center) comparisons to state-of-the-art image inpainting.}
Results are generated using open-source code and pre-trained models from the original authors.
All examples are randomly selected.}
\label{fig:places2_randomly_0}
\end{figure}

==> figures/comparisons/places2_1.tex <==
\begin{figure}[!ht]
\centering
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/places2/input/8566.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/input/15053.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/input/15749.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/input/1410.png}
\caption{Input}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/places2/gated_conv/8566.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/gated_conv/15053.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/gated_conv/15749.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/gated_conv/1410.png}
\caption{GatedConv \cite{GatedConvolutionYu}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/places2/plurastic_inpainting/8566.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/plurastic_inpainting/15053.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/plurastic_inpainting/15749.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/plurastic_inpainting/1410.png}
\caption{PIC \cite{zheng2019pluralistic}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/places2/result/8566.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/result/15053.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/result/15749.png}
\includegraphics[width=\textwidth]{images/comparisons/places2/result/1410.png}
\caption{Ours}
\end{subfigure}%%
\caption{
\textbf{Places2 (Center) comparisons to state-of-the-art image inpainting.}
Results are generated using open-source code and pre-trained models from the original authors.
All examples are randomly selected.}
\label{fig:places2_randomly_1}
\end{figure}

==> figures/comparisons/places2_free_form_0.tex <==
\begin{figure}[!ht]
\centering
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/input/14923.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/input/28540.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/input/31349.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/input/34526.png}
\caption{Input}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/gated_conv/14923.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/gated_conv/28540.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/gated_conv/31349.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/gated_conv/34526.png}
\caption{GatedConv \cite{GatedConvolutionYu}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/plurastic_inpainting/14923.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/plurastic_inpainting/28540.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/plurastic_inpainting/31349.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/plurastic_inpainting/34526.png}
\caption{PIC \cite{zheng2019pluralistic}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/result/14923.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/result/28540.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/result/31349.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/result/34526.png}
\caption{Ours}
\end{subfigure}%%
\caption{
\textbf{Places2 (Free-Form) comparisons to state-of-the-art image inpainting.}
Results are generated using open-source code and pre-trained models from the original authors.
All examples are randomly selected.}
\label{fig:places2_free_form_randomly_0}
\end{figure}

==> figures/comparisons/places2_free_form_1.tex <==
\begin{figure}[!ht]
\centering
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/input/29145.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/input/712.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/input/20702.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/input/23534.png}
\caption{Input}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/gated_conv/29145.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/gated_conv/712.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/gated_conv/20702.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/gated_conv/23534.png}
\caption{GatedConv \cite{GatedConvolutionYu}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/plurastic_inpainting/29145.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/plurastic_inpainting/712.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/plurastic_inpainting/20702.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/plurastic_inpainting/23534.png}
\caption{PIC \cite{zheng2019pluralistic}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/result/29145.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/result/712.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/result/20702.png}
\includegraphics[width=\textwidth]{images/comparisons/places2_free_form/result/23534.png}
\caption{Ours}
\end{subfigure}%%
\caption{
\textbf{Places2 (Free-Form) comparisons to state-of-the-art image inpainting.}
Results are generated using open-source code and pre-trained models from the original authors.
All examples are randomly selected.}
\label{fig:places2_free_form_randomly_1}
\end{figure}

==> figures/comparisons/pluralistic_0.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/masked_out/1.png}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/masked_out/2.png}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/masked_out/3.png}
\caption{Input}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/gated_conv/1.png}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/gated_conv/2.png}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/gated_conv/3.png}
\caption{GConv \cite{GatedConvolutionYu}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/pluralistic/1.png}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/pluralistic/2.png}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/pluralistic/3.png}
\caption{PIC \cite{zheng2019pluralistic}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/result/1.png}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/result/2.png}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/result/3.png}
\caption{Ours}
\end{subfigure}%%
\caption{\textbf{CelebA-HQ comparison to state-of-the-art models}
Examples selected by authors of \cite{zheng2019pluralistic} (images extracted from their paper and supplementary material).
Due to the original images and masks being stored in .jpg format with compression, the results might differ from original paper.
Therefore, we decided to generate results from \cite{zheng2019pluralistic} again.
Results of \cite{GatedConvolutionYu,zheng2019pluralistic} generated by using their open-source code and models.
Note that the original image size is $256 \times 256$.
We recommend the reader to zoom-in on missing regions.}
\label{fig:pluralistic_0}
\end{figure}

==> figures/comparisons/pluralistic_1.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/masked_out/4.png}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/masked_out/5.png}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/masked_out/6.png}
\caption{Input}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/gated_conv/4.png}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/gated_conv/5.png}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/gated_conv/6.png}
\caption{GConv \cite{GatedConvolutionYu}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/pluralistic/4.png}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/pluralistic/5.png}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/pluralistic/6.png}
\caption{PIC \cite{zheng2019pluralistic}}
\end{subfigure}%%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/result/4.png}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/result/5.png}
\includegraphics[width=\textwidth]{images/comparisons/pluralistic/celebA_HQ/result/6.png}
\caption{Ours}
\end{subfigure}%%
\caption{\textbf{CelebA-HQ comparison to state-of-the-art models}
Examples selected by authors of \cite{zheng2019pluralistic} (images extracted from their paper and supplementary material).
Due to the original images and masks being stored in .jpg format with compression, the results might differ from original paper.
Therefore, we decided to generate results from \cite{zheng2019pluralistic} again.
Results of \cite{GatedConvolutionYu,zheng2019pluralistic} generated by using their open-source code and models.
Note that the original image size is $256 \times 256$.
We recommend the reader to zoom-in on missing regions.}
\label{fig:pluralistic_1}
\end{figure}

==> figures/deterministic/full.tex <==
\begin{figure}
\centering
\includegraphics[width=\textwidth]{images/deterministic/full.png}
\caption{
\textbf{Diverse Plausible Results:}
Images from the FDF validation dataset \cite{hukkelaas2019DeepPrivacy}.
Left column is the input image with the pose information marked in red.
Second column and onwards are different plausible generated results.
Each image is generated by randomly sampling a latent variable for the generator (except for the second column where the latent variable set to all 0's)}
\label{fig:deterministc_experiment_appendix}

\end{figure}

==> figures/deterministic/random.tex <==
\begin{figure}
\centering
\includegraphics[width=\textwidth]{images/deterministic/random.png}
\caption{
\textbf{Diverse Plausible Results (Randomly Selected):}
Images from the FDF validation dataset \cite{hukkelaas2019DeepPrivacy}.
Left column is the input image with the pose information marked in red.
Second column and onwards are different plausible generated results.
Each image is generated by randomly sampling a latent variable for the generator (except for the second column where the latent variable set to all 0's).
All images are randomly selected.}
\label{fig:deterministc_experiment_appendix_random}

\end{figure}

==> figures/main_qualitative.tex <==
\begin{figure}
\centering
%\includegraphics[width=\textwidth]{}
\caption{
\textbf{A bunch of really good results !}}
\label{fig:main_qualitative}
\end{figure}

==> figures/train_graph.tex <==
\begin{figure}[H]
    \centering
    \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{images/ICONV_comparison_small.png}
%    \caption{Pconv \cite{PconvLiu}}
    \end{subfigure}
    \hspace{.01\textwidth}
    \begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{images/ICONV_comparison_walltime_small.png}
%    \caption{Gated Conv \cite{GatedConvolutionYu}}
    \end{subfigure}
    \caption{LPIPS \cite{zhang2018perceptual} improvement during training our model with and without IConv for Places 2.}
    \label{fig:training_graph}
\end{figure}


==> tables/densepose_table.tex <==

\begin{table}
	\caption{
		Fr\`echet Inception Distance (FID) on the FDF validation set with and without mask extracted from DensePose (lower is better).
		We report FID after showing the discriminator 12M images.
	}
	\centering
	
	\begin{tabular}{c|c|c}
		\hline
		Mask Type & 12M & 20M \\
		\hline
		Original FDF \cite{hukkelaas2019deepprivacy} & 4.36  & 2.94 \\
		FDF + DensePose Mask & 3.64 & 2.29\\
		
		\hline
	\end{tabular}
	\label{tab:densepose_table}
\end{table}

==> tables/full_config_table.tex <==
\begin{table}
\caption{
	Quantitative results on the FDF dataset \cite{hukkelaas2019DeepPrivacy}.
	We report standard metrics after showing the discriminator 20M images.
	* Did not converge.
	$\dagger$ Same as Config B.}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{ll|cccccc|cccccc}
	\hline
	\multicolumn{2}{l|}{Configuration} & \multicolumn{6}{c|}{FDF \cite{hukkelaas2019DeepPrivacy}} & \multicolumn{6}{c}{Places2 \cite{places2}} \\ 
	\hline
 &  & LPIPS $\downarrow$ & PSNR $\uparrow$ & FID $\downarrow$ & L1 $\downarrow$ & L2 $\downarrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & FID $\downarrow$ & L1 $\downarrow$ & L2 $\downarrow$ & SSIM $\uparrow$ \\

	A &  Baseline \cite{hukkelaas2019DeepPrivacy} & 22.52 & 0.1036 & 6.16 & 0.03 & 0.08 & 0.756 & --* & --* & --* & --* & --* & --* \\
B &  + Improved Gradient penalty & 0.0757 & 23.92 & 1.83 & 0.03 & 0.07 & 0.787 & 0.1619 & 20.99 & 7.96 & 0.03 & 0.10 & 0.747 \\
C & + Scalar Pose Information & 0.0733 & 24.01 & 1.76 & 0.02 & 0.07 & 0.791 & --$\dagger$ & --$\dagger$ & --$\dagger$ & --$\dagger$ & --$\dagger$ & --$\dagger$ \\
D & + Learned Pool & 0.0739 & 23.95 & 1.66 & 0.03 & 0.07 & 0.790 & 0.1563 & 21.21 & 6.81 & 0.03 & 0.10 & 0.749 \\
\hline
E & + No Growing, MSG & 0.0728 & 24.01 & 1.49 & 0.02 & 0.07 & 0.790 & 0.1491 & 21.42 & 5.24 & 0.03 & 0.10 & 0.752 \\


\end{tabular}}
\label{tab:configurations_full}
\end{table}


==> tables/gradient_penalty.tex <==
\begin{table}
	
	\caption{
		Fr\`echet Inception Distance (FID) on the FDF validation set for a different set of gradient penalty functions (lower is better).
		We report FID after showing the discriminator 12M  and 18M images.
		The hyperparameters and model size is the same for each model.
		*The experiment diverged or collapsed before reaching 12M images.
	}
	\centering
	
	\begin{tabular}{c|c|c}
		\hline
		Gradient Penalty ($g(\hat{x})$) & 12M & 18M \\
		\hline
		$(||\nabla D(\hat{x})||_2 -1 )^2$ & $2.45$  & $97$\\
		$\max(0,||\nabla D(\hat{x})||_2 -1)$ & $2.56$ & \textbf{1.63}\\
		\cline{0-0}
		$(||\nabla D(\hat{x}) \odot (1-M)||_2 -1 )^2$ & --* & --* \\
		$\max(0,||\nabla_{\hat{x}} D(\hat{x}) \odot (1-M)||_2 -1)$ & --* & --* \\
		\hline 
		$(||\nabla D(\hat{x})||_\infty -1 )^2$ &  $2.52$ & $1.75$\\
		$\max(0, ||\nabla D(\hat{x})||_\infty -1)$ & 2.17 & 1.39\\
		\cline{0-0}
		$(||\nabla D(\hat{x})\odot (1-M)||_\infty -1 )^2$ &  $2.47$ & $1.64$\\
		$\max(0, ||\nabla D(\hat{x})\odot (1-M)||_\infty -1)$ & \textbf{2.17} & \textbf{1.34}\\		
			
		\hline
	\end{tabular}
	\label{tab:gradient_penalty}
\end{table}


==> tables/gradient_penalty_comparison.tex <==
\begin{table}[t]
	
\caption{
	\textbf{Quantitative results of the impact of different gradient penalties}
	Quantitative results on the FDF dataset \cite{hukkelaas2019DeepPrivacy}.
	We report FID and LPIPS after showing the discriminator 30M images for Config A-D.
	For Config E, we report after showing the discriminator 20M images.
	*The training collapsed before reaching 30M images.
}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc|cc}
	\hline
	\multirow{2}{*}{Gradient Penalty} & \multicolumn{2}{|c|}{Config A} & \multicolumn{2}{|c|}{Config B} & \multicolumn{2}{|c|}{Config C} & \multicolumn{2}{|c|}{Config D} & \multicolumn{2}{|c|}{Config E} \\
	 & FID & LPIPS (\%) & FID & LPIPS (\%) & FID & LPIPS (\%) & FID & LPIPS (\%) & FID & LPIPS (\%) \\
	\hline
	$L^2$ & 4.38 & 9.66 & 2.81 & 7.96 & \textbf{1.53} & \textbf{7.25} & \textbf{1.43} & \textbf{7.15} & \textbf{1.61} & \textbf{8.07} \\
	
	$L^\infty$ & --* & --* & \textbf{1.90} & \textbf{7.67} & 1.61 & 7.28 & 1.56 & 7.23 & 1.67 & 8.08 \\
	\hline

\end{tabular}}
\label{tab:gradient_penalty_comparison}
\end{table}


==> tables/pconv_table.tex <==
\begin{table}
	
	\caption{
		Fr\`echet Inception Distance (FID) on the FDF validation set for a different set of gradient penalty functions (lower is better).
		We report FID after showing the discriminator 20M  and 30M images.
		The hyperparameters and model size is the same for each model.
	}
	\centering
	\begin{tabular}{l|c|c}
		\hline
		Configuration & 20M & 30M \\
		\hline
        Config D & 1.77 & 1.38 \\
        \hline
        Config D + Weighted Pool & 2.00 & 1.44 \\ 
        \hline
        Config D + Learned Pool & \textbf{1.53} & \textbf{1.18} \\
		\hline
	\end{tabular}
	\label{tab:pconv_table}
\end{table}

